Gaussian Processes for Surrogate Modeling of Discharged Fuel Nuclide Compositions

Several applications such as nuclear forensics, nuclear fuel cycle simulations and sensitivity analysis require methods to quickly compute spent fuel nuclide compositions for various irradiation histories. Traditionally, this has been done by interpolating between one-group cross-sections that have been pre-computed from nuclear reactor simulations for a grid of input parameters, using fits such as Cubic Spline. We propose the use of Gaussian Processes (GP) to create surrogate models, which not only provide nuclide compositions, but also the gradient and estimates of their prediction uncertainty. The former is useful for applications such as forward and inverse optimization problems, the latter for uncertainty quantification applications. For this purpose, we compare GP-based surrogate model performance with Cubic- Spline-based interpolators based on infinite lattice simulations of a CANDU 6 nuclear reactor using the SERPENT 2 code, considering burnup and temperature as input parameters. Additionally, we compare the performance of various grid sampling schemes to quasirandom sampling based on the Sobol sequence. We find that GP-based models perform significantly better in predicting spent fuel compositions than Cubic-Spline-based models, though requiring longer computational runtime. Furthermore, we show that the predicted nuclide uncertainties are reasonably accurate. While in the studied two-dimensional case, grid- and quasirandom sampling provide similar results, quasirandom sampling will be a more effective strategy in higher dimensional cases.

==> Paper GPR - Annals of Nuclear Energy (Publishing)/Sections/Abstract.tex <==
\begin{abstract}
     Several applications such as nuclear forensics, nuclear fuel cycle simulations and sensitivity analysis require methods to quickly compute spent fuel nuclide compositions for various irradiation histories. Traditionally, this has been done by interpolating between one-group cross-sections that have been pre-computed from nuclear reactor simulations for a grid of input parameters, using fits such as Cubic Spline. We propose the use of Gaussian Processes (GP) to create surrogate models, which not only provide nuclide compositions, but  also the gradient and estimates of their prediction uncertainty. The former is useful for applications such as forward and inverse optimization problems, the latter for uncertainty quantification applications. For this purpose, we compare GP-based surrogate model performance with Cubic-Spline-based interpolators based on infinite lattice simulations of a CANDU 6 nuclear reactor using the \texttt{SERPENT 2} code, considering burnup and temperature as single dimensional input parameters resulting in a 2D study. Additionally, we compare the performance of uniform grid sampling to quasirandom sampling based on the Sobol sequence. We find that GP-based models perform significantly better in predicting spent fuel compositions than Cubic-Spline-based models on both sampling schemes. Uniform grid sampling performs better than quasirandom sampling in our 2D study, this cannot be generalized to higher dimensions. We have found that GP models require more time to compute a prediction. Although a relatively small time ($\mathcal{O}$ ms), iterative methods used for statistical inference benefit from from as-low-as-possible calculation times. Furthermore, we show that the predicted nuclide uncertainties are reasonably accurate. While in the studied two-dimensional case, grid- and quasirandom sampling provide similar results, quasirandom sampling will be a more effective strategy in higher-dimensional cases.
    
    
    
    
\end{abstract}

%\section*{Online submitted abstract}
%Several applications such as nuclear forensics, nuclear fuel cycle simulations and sensitivity analysis require methods to quickly compute spent fuel nuclide compositions for various irradiation histories. 
%Traditionally, this has been done by interpolating precomputed one-group cross-sections obtained from nuclear reactor simulations on a grid of input parameters, using fits such as Cubic Spline. We propose the use of Gaussian Processes (GP) to create surrogate models, which not only provide nuclide compositions, but also the gradient and estimates of their prediction uncertainty. 
%For this purpose, we compare GP-based surrogate model performance with Cubic-Spline-based interpolators based on infinite lattice simulations of a CANDU-6 nuclear reactor using the SERPENT 2 code, considering burnup and temperature as input parameters. 
%We find that GP-based models have higher performance in predicting spent fuel compositions than Cubic-Spline-based models, though requiring longer computational runtime. Furthermore, we show that the predicted nuclide uncertainties are reasonably accurate and reliable. 

==> Paper GPR - Annals of Nuclear Energy (Publishing)/Sections/Acknowledgements.tex <==
\section*{Acknowledgments}
This research was funded by the Mathematics Division of the Center for Computational Engineering Science at RWTH Aachen University, and the Volkswagen Foundation. We would like to thank Manuel Torrilhon for his support. The funding sources had no role in the study design, collection, analysis and interpretation of data as well in the writing of the report. The calculations were run on RWTH Aachen's Compute Cluster under the rwth0572 project.

==> Paper GPR - Annals of Nuclear Energy (Publishing)/Sections/Conclusion.tex <==
\section{Conclusion}\label{section:conclusion}
We have compared two interpolation methods for direct fast prediction of spent fuel nuclide compositions. As expected, GP models typically require significantly more time to interpolate values. While the time itself is of the order of miliseconds for a relatively small training set size, for large-scale applications involving a very large number of calculations for many nuclides, as is for instance the case when solving Bayesian inference problems using Markov Chain Monte Carlo \cite{ESARDA-Antonio}, it is desired to keep the required calculation time as low as possible. In return for this larger calculation time, GP models provide an estimate of the prediction uncertainty as well as an explicit method for estimating the gradient of the underlying function, provided the kernels used are differentiable. This can be useful for the solution of both forward and inverse optimization problems. 

Additionally, we have noted that GP models result in smaller interpolation errors under the $RMSE$ metric, with varying reduction factors of up to 20 when compared to Cubic Spline interpolation. % This varies depending on the experimental design used, however, a difference between the use of Sobol to uniform Grid sampling was observed, being that models trained on the latter perform better than those trained on the former, for both Spline and GP based models. We expect however, that the use of Sobol sampling for higher dimensional problems would outperform the results obtained from Grid-based methods. 

Several possibilities exist for the extension of this work. As of now, we have created GP models depending only on two input parameters using the ASE kernel. Future research could entail the inclusion of a larger number of parameters such as power or reactor downtime, as well as the use of different kernels and even combinations of kernels for more flexible models. %Recent research on multi model kriging could be useful for the determination and selection of the kernels to use.

Higher fidelity GP models can be created by the use of 3-D full core reactor simulations, to account for spatial variation of nuclide concentrations and burnup, temperature and power levels. Building such GP-based models would, however, be significantly more computationally expensive. 

As we have only studied GPR to directly predict isotopic compositions, a further research area could be the study of the predictive performance when implementing GPR on a cross-section level. This could enable implementing changes in the model parameters during the irradiation cycle. This approach could make feasible the forward uncertainty estimation via Monte Carlo methods, calculating the nuclide concentrations through the matrix exponential method, all thanks to the predictive variance of the interpolated one-group cross-sections.

In conclusion, we hope that the full potential of GP-based modelling of nuclear processes will be further studied and exploited in the future, having discussed here the many advantages it has for nuclear engineering applications.




==> Paper GPR - Annals of Nuclear Energy (Publishing)/Sections/DataAvailability.tex <==
\section*{Data Availability}
The code used for the implementation of GP models and their comparison with Cubic Spline models can be obtained at:
\url{https://github.com/FigueroaAC/GPs-for-SpentFuel}
%\url{https://bit.ly/3dplFLC}

==> Paper GPR - Annals of Nuclear Energy (Publishing)/Sections/Introduction.tex <==
\section{Introduction}

The computation of spent fuel nuclide compositions is a complex problem which involves  modelling the fuel assembly, reactor geometries and tracking the nuclide evolution as the fuel is irradiated following an operational history indicated by different parameters such as burnup, power, and temperature. This requires the numerical solution of the neutron transport equation through probabilistic - namely Monte Carlo calculations - or deterministic methods \cite{nuchb}, which are computationally expensive. 

For several applications however, it is desirable to have a fast and computationally less intensive method to compute nuclide compositions, especially when many repeated calculations are needed for further analysis. Examples of this are nuclear fuel cycle simulators \cite{cyclus}, nuclear forensics applications \cite{forensics}, and sensitivity analyses, the latter illustrated by \cite{sensitivity} where it is performed for a model which discriminates reactor types based on measurements of plutonium samples and their errors.

This problem has been addressed in the past through pre-computed data-bases of reactor simulations, and the interpolation of either the one-group cross-sections \cite{arp} \cite{cyclus2} or nuclide concentrations resulting from these simulations with different methods such as: Nearest Neighbors, Linear Fit, Lagrange Polynomials, Neural Networks \cite{baptiste}, and Cubic Splines, the latter being currently the most commonly used.

Up until now, most of the available software packages have used infinite lattice reactor simulations sampled on a uniform multi-dimensional grid of at most three dimensions \cite{arp}\cite{cyclus2}. For low dimensional problems ($d\leq3$), uniform grid sampling produces good results, however for a larger number of dimensions, this sampling method does not distribute the sampling points efficiently across space \cite{DOE}, resulting in poor exploration of the parameter space. Quasirandom Sampling methods would provide better space coverage properties at higher dimensions \cite{DOE}. However, some of the above mentioned interpolation methods require the samples to be distributed on a grid in order to perform correctly. Furthermore, while the interpolation quality can be estimated, the aforementioned interpolation methods do not provide information on the expected variance of the interpolation at non-sampled points. 

Here, we propose using Gaussian Processes (GP) for interpolation, by considering noiseless inputs. Under this assumption, GP's provide zero error on points arising from the dataset on which the models have been trained, whereas a regression is performed for unseen data points. In addition, this method has already been used in conjunction with Quasirandom Sampling \cite{ESARDA-Antonio}. Furthermore, also the gradient and estimates of their prediction uncertainty at non-sampled points are directly obtained. The former is useful for applications such as forward and inverse optimization problems, the latter for uncertainty quantification applications. GP belongs to a set of tools used in the Machine Learning communities for a variety of tasks, including classification and regression. With Gaussian Process Regression (GPR), the interpolation is not performed on a specific function but over an infinite distribution of functions that share common properties as defined by the user.

An equivalent concept to GPR called kriging is well known in the field of geology \cite{recipes}. Recently, researchers have used GP-based surrogate models for nuclear engineering applications such as modeling of equipment degradation and preventive maintenance \cite{degradation}, or studying fuel performance and thermo-hydraulics \cite{BayesGP}. They also have been used for the prediction of fuel nuclide compositions and compared to surrogate models based on Dynamic
Mode Decomposition, by performing regression on a Principal Component Analysis (PCA) model of the fuel isotopics \cite{dmd}. Additionally, we have started exploring  their use for the direct prediction of spent fuel compositions, without a PCA-reduced model and using multidimensional input variables \cite{ESARDA-Antonio}, work that we update here
 

In this paper, we compare the performance of GP-based surrogate models to models based on Cubic Splines for the direct interpolation of spent fuel nuclide compositions (GP could also interpolate cross-sections). We compare to Cubic Splines as they often produce smoother and higher quality interpolators in comparison to methods such as Langrange and Newton polynomials \cite{na}. The performance of both techniques will be explored through computational experiments involving different sampling configurations using both Grid sampling and Sobol Quasirandom Sequences in order to assess the impact of the sampling strategy on the regressions. We study two-dimensional problems to examine whether GPR performs well already in problems where grid sampling is still effective.

==> Paper GPR - Annals of Nuclear Energy (Publishing)/Sections/Results.tex <==
\section{Results and Discussion}\label{section:results}
We have compared GPR-based models of spent fuel nuclide concentrations to Cubic Splines models of these quantities. The Splines models have been implemented using the \texttt{SmoothBivariateSpline} module from the \texttt{Scipy} \cite{scipy} python package. The following comparison is focused on two main elements: Runtime Performance and Model Quality. 

\subsection{Runtime performance}
We have studied the mean time required to perform a prediction for the interpolation methods discussed in this article. This calculation time we refer to here as \textit{runtime} is different from the time required to train the model which in itself is dependent on the sample size, the number of dimensions and the subsequent optimization problem that is to be solved in order to derive the appropriate kernel hyperparameters. The tests have been performed on a 2.2 GHz \texttt{Intel Core i7} computer with 4 cores and 16GB of RAM. Table \ref{tab:runtime} shows the regression time required averaged over all the models, with the time for a GP model separated into the time required for the prediction \textbf{GPR}$-\mu$ and the time required for the estimation of the prediction variance \textbf{GPR}$-\sigma$, as these calculations can be run independently of each other.

%While in our implementation they are calculated sequentially, the values shown in this table indicate that the time required for prediction and variance estimation is similar, thus hinting at a potential total runtime reduction by a factor of 2. Nevertheless, 
Interpolation using GP models can require significantly more time than interpolation based on Cubic Splines. It might be possible that through the use of more efficient implementations, the runtime difference between the two can be reduced in the future.

\input{Sections/Tables/tableruntime}

\subsection{Model Quality}
We have analyzed the quality of the models based on GP's and Cubic Splines using the experimental designs presented in Table \ref{tab:setups} and Figures \ref{fig:SvG} and \ref{fig:exppatterns}. For this, we have considered an array of metrics to quantify model performance, namely the root-mean-square-errors ($RMSE$) and the coefficients of determination $R^{2}$. We also examine an additional metric related to the posterior predictive variance produced by GPR in order to study the quality of this estimator. This quantity is $Pred-1\sigma$, which quantifies the fraction of model predictions located within 1 predictive standard deviation from the true values of the test sets, i.e. it shows whether the predicted variance represents the variance that is actually observed. 

While models were created for each of the nuclides tracked by \texttt{SERPENT 2}, Tables %\ref{res:checkerboard}, \ref{res:sobol}, \ref{tab:grid2}, and \ref{res:grid4}  
\ref{tab:grid2} and \ref{tab:sobolnew} contain the results of
our analysis for a small subset of them representative of both major actinides and fission products. The mean values shown have been scaled by the assembly length and number of fuel assemblies in the reactor core. 
\input{Sections/Tables/tablegrid2}
\input{Sections/Tables/tablesobolnew}

In general, we observe that based on the $R^{2}$ metric, both interpolation methods have good performance for most of the nuclides. Furthermore, we note that based on the $RMSE$ metric, GP based models perform  better in all the experimental configurations for all isotopes. The improvement of the mean RMSE is in most cases between a factor of 1.02 and 10. Still, Cubic Splines could provide on average reasonable results for most nuclides, provided the application requirements allow for $RMSE$ errors of such magnitude.

 %This phenomenon has been observed on both models based on the uniform grid and the Sobol sequence. A possible cause of this might be in the specific shape of these curves, specifically in the case of $^{147}$ Nd where a non monotonic shape can be observed. A closer inspection of the raw data reveals oscillations in these curves, an explanation for which might be that both of these nuclides have very large absorption cross-sections, especially in the thermal and epithermal regions of the energy spectrum, so small perturbations in the flux can potentially have large effects on the nuclide concentrations. In our computer experiments this translates into numerical perturbations resulting in significative effects on the nuclide concentrations. 

%We believe that in this case Cubic Splines have problems interpolating such perturbations in the model outputs, whereas in the case of GP models, the result is a regression to the mean with relatively large posterior uncertainties, as can be observed in figures \ref{fig:Nd147} and \ref{fig:Sm151} where we show curves generated from the raw data of reactor simulations with their respective Cubic Spline and GP models. A different result, for example in the case of $^{239}$Pu \ref{fig:gpr_model} can be seen, in which the prediction uncertainties can be very small as the raw data does not result in intersecting curves.

%\begin{figure}[ht!]
%    \centering
% \input{Sections/Images/Nd147}
% \vspace{150pt}
%        \caption{Top to bottom and left to right: Raw data from simulations, Cubic Spline Model, GP Model for $^{147}$Nd. In the raw data figure, a portion has been zoomed in to show the crossing curves, each corresponding to a different temperature. The shape of the curve and these perturbations might complicate models based on Cubic Splines, and increase uncertainties on GP models predictions. The models shown have been built from the Sobol sequence dataset.}
%    \label{fig:Nd147}
%\end{figure}

%\begin{figure}[ht!]
%    \centering
% \input{Sections/Images/Sm151}
% \vspace{150pt}
%        \caption{Top to bottom and left to right: Raw data from simulations, Cubic Spline Model, GP Model for $^{151}$Sm. In the raw data figure, a portion has been zoomed in to show the crossing curves, each corresponding to a different temperature. The shape of the curve and these perturbations might complicate models based on Cubic Splines, and increase uncertainties on GP models predictions. The models shown have been built from the Sobol sequence dataset.}
%    \label{fig:Sm151}
%\end{figure}

%\begin{figure}
%    \centering
% \input{Sections/Images/Xe135}
% \vspace{150pt}
%        \caption{Top to bottom and left to right: Raw data from simulations, Cubic Spline Model, GP Model for $^{135}$Xe. In the raw data figure, a portion has been zoomed in to show the crossing curves, each corresponding to a different temperature. The shape of the curve and these perturbations might complicate models based on Cubic Splines, and increase uncertainties on GP models predictions. The models shown have been built from the Sobol sequence dataset.}
%    \label{fig:Xe135}
%\end{figure}


% Interestingly we have observed that GPR also has problems interpolating $^{147}$Nd when implemented over the grid with spacing of 4 units. We believe that in this case, the reason might be the low spatial density of the training design, resulting in a very smooth interpolation, missing the fluctuations in the nuclide concentration. In practice this can be solved by increasing the global sampling density or locally if prior information about the distribution of concentrations is known.

%This being said, 
We also observe that the variance predictor of the GP model predicts the true values at the $1-\sigma$ level reasonably well, which is not generalizable to any GPR application. In addition,it can be seen that both surrogate model methods perform better on a uniform grid-based sample set compared to a sampled set based on Sobol sequences. Nevertheless, based on a study where different sampling schemes are compared for their space covering properties and efficiency \cite{DOE}, one would expect the positive properties of Sobol sequences to be made manifest in problems of higher dimensionality.



%\subsection{Sensitivity Analysis}

% Not sure about this, as most of the isotopes are globally sensible only to Burnup.
%\begin{table}[ht]
 %   \centering
  %  \begin{tabular}{c c c c }\toprule
    %\textbf{Nuclide} & $B>T$ & 
    %$T>B$ & $B\approx T$\\ \midrule
   %$^{239}$Pu & \checkmark & -& - \\
         %$\vdots$ &$\vdots$ %&$\vdots$ &$\vdots$ \\ 
%         & & & \\
         
   %\bottomrule
     
    %\end{tabular}
    %\caption{Relative nuclide sensitivity to input parameter, based on AES kernel. $T$ and $B$ stand for Temperature and Burnup %respectively}
%    \label{tab:sensitivity}
%\end{table}

==> Paper GPR - Annals of Nuclear Energy (Publishing)/Sections/Sections/Images/Pu2d.tex <==
	\newcommand{\dsurfPu}{Sections/Images/2dSobolPu239.csv}
	\newcommand{\dsurfPuN}{Sections/Images/Pu2392dComplement.csv}	
	\begin{axis}[name = surf,
		%at=(collapsed.right of south east) ,anchor=left of south west,
		smooth,
		legend pos = north east,
		%mark repeat=10,%
		colormap/greenyellow,
		xlabel = {\textbf{Temperature} ($K$ )},
		ylabel = \textbf{Burnup} $\frac{\mathrm{MWd}}{\mathrm{KgHM}}$,
		zlabel = \textbf{Mass} (Kg),
		xlabel style={rotate=-9},
		ylabel style={rotate=35},  title= $^{239}$\textbf{Pu}
		%y label/.append style={at=(ticklabel* cs:0)},
		%zlabel style={anchor=south west},] %
		]
		\addplot3 [surf,z buffer=sort, mesh/rows=25, opacity=0.6]
		table[y={Burnup}, x={Temperature} , z={Pred}, col sep=comma] {\dsurfPu};
		\addplot3+[only marks, scatter] table[y={Burnup}, x={Temperature} , z={Yts}, col sep=comma] {\dsurfPuN};
	\end{axis} %

==> Paper GPR - Annals of Nuclear Energy (Publishing)/Sections/Tables/tablecheckerboard.tex <==

\begin{table}[ht!]
\centering
	\resizebox{\tablesize\textwidth}{!}{
		\pgfplotstabletypeset[
		multicolumn names, % allows to have multicolumn names
		col sep=comma, % the seperator in our .csv file
		columns = {Nuclide,mean_isotope,Spline-RMSE,GPR-RMSE,RatioCubicGPR,SplineRsquared,GPRRsquared,GPRPredictionin1sigma},
		columns/Nuclide/.style={
			column name=$Nuclide$, % name of first column
			string type},  % use siunitx for formatting
		columns/mean_isotope/.style={
			column name=$\mu$, % name of first column
			precision=2,fixed}, 
		columns/Spline-RMSE/.style={
			column name= Cubic Spline,
			string type},
		columns/GPR-RMSE/.style={
			column name=$GPR$,string type},
		columns/RatioCubicGPR/.style={
		column name=RMSE $\frac{Spline}{GPR}$,
		precision=2},
		columns/SplineRsquared/.style={
			column name=$R^{2}_{Sp}$,
			%sci, sci zerofill,
			precision=2},%, sci 10e},
		columns/GPRRsquared/.style={
			column name=$R^{2}_{GPR}$,
			%sci, sci zerofill,
			precision=2},%, sci 10e},
		columns/GPRPredictionin1sigma/.style={
			column name=$Pred-1\sigma$,
			precision=1,},
		%display columns/8/.style={
		%	column name=$Pred-2\sigma$,
		%	precision=1,},
		every head row/.style={
			before row={\toprule}, % have a rule at top
			after row={
							&	Kg& $\mathrm{RMSE}$ & $\mathrm{RMSE}$  & &  & & $\%$ \\% & $\%$ \\ % the units seperated by &
				\midrule} % rule under units
		},
		every last row/.style={after row=\bottomrule}, % rule at bottom
		]{Sections/Tables/Checkerboard_all_2space.csv} % filename/path to file
		}
			\caption{Comparison between GPR and Cubic spline models for a selection of nuclides. The models have been trained on a squared grid with a Checkerboard arrangement. Highlighted cells indicate smallest error in the comparison. RMSE values are in Kg}
        \label{res:checkerboard}
\end{table}


==> Paper GPR - Annals of Nuclear Energy (Publishing)/Sections/Tables/tablegrid2.tex <==
\begin{center}
\begin{table*}[ht!]
\centering
	\resizebox{\tablesize\textwidth}{!}{
		\pgfplotstabletypeset[
		multicolumn names, % allows to have multicolumn names
		col sep=comma,
		columns = {Nuclide,mean_isotope,Spline-RMSE,GPR-RMSE,RatioCubicGPR,SplineRsquared,GPRRsquared,GPRPredictionin1sigma},
		columns/Nuclide/.style={
			column name=$Nuclide$, % name of first column
			string type},  % use siunitx for formatting
		columns/mean_isotope/.style={
			column name=$\mu$, % name of first column
			precision=2,fixed}, 
		columns/Spline-RMSE/.style={
			column name= Cubic Spline,
			string type},
		columns/GPR-RMSE/.style={
			column name=$GPR$,string type},
		columns/RatioCubicGPR/.style={
		column name=RMSE $\frac{Spline}{GPR}$,
		precision=2},
		columns/SplineRsquared/.style={
			column name=$1 - R^{2}_{Sp}$,
			%sci, sci zerofill,
			string type},%, sci 10e},
		columns/GPRRsquared/.style={
			column name=$1 - R^{2}_{GPR}$,
			%sci, sci zerofill,
			string type},%, sci 10e},
		columns/GPRPredictionin1sigma/.style={
			column name=$Pred-1\sigma$,
			precision=1,},
		every head row/.style={
			before row={\toprule}, % have a rule at top
			after row={
							&	Kg& $\mathrm{RMSE}$ & $\mathrm{RMSE}$  & &  & & $\%$ \\%& $\%$ \\ % the units seperated by &
				\midrule} % rule under units
		},
		every last row/.style={after row=\bottomrule}, % rule at bottom
		]{Sections/Tables/Even_all_2space.csv} % filename/path to file
		}
			\caption{\textbf{Scenario A:} Comparison between GPR and Cubic spline models for a selection of nuclides. Highlighted cells indicate smallest error in the comparison. RMSE values are in Kg}
			\label{tab:grid2}
\end{table*}
\end{center}

==> Paper GPR - Annals of Nuclear Energy (Publishing)/Sections/Tables/tablegrid4.tex <==

\begin{table}[ht!]
\centering
    \resizebox{\tablesize\textwidth}{!}{
		\pgfplotstabletypeset[
		multicolumn names, % allows to have multicolumn names
		col sep=comma, % the seperator in our .csv file
		columns = {Nuclide,mean_isotope,Spline-RMSE,GPR-RMSE,RatioCubicGPR,SplineRsquared,GPRRsquared,GPRPredictionin1sigma},
		columns/Nuclide/.style={
			column name=$Nuclide$, % name of first column
			string type},  % use siunitx for formatting
		columns/mean_isotope/.style={
			column name=$\mu$, % name of first column
			precision=2,fixed}, 
		columns/Spline-RMSE/.style={
			column name= Cubic Spline,
			string type},
		columns/GPR-RMSE/.style={
			column name=$GPR$,string type},
		columns/RatioCubicGPR/.style={
		column name=RMSE $\frac{Spline}{GPR}$,
		precision=2},
		columns/SplineRsquared/.style={
			column name=$R^{2}_{Sp}$,
			%sci, sci zerofill,
			precision=2},%, sci 10e},
		columns/GPRRsquared/.style={
			column name=$R^{2}_{GPR}$,
			%sci, sci zerofill,
			precision=2},%, sci 10e},
		columns/GPRPredictionin1sigma/.style={
			column name=$Pred-1\sigma$,
			precision=1,},
		every head row/.style={
			before row={\toprule}, % have a rule at top
			after row={
							&	Kg& $\mathrm{RMSE}$ & $\mathrm{RMSE}$  & &  & & $\%$ \\%& $\%$ \\ % the units seperated by &
				\midrule} % rule under units
		},
		every last row/.style={after row=\bottomrule}, % rule at bottom
		]{Sections/Tables/Even_all_4space.csv} % filename/path to file
		}
			\caption{Comparison between GPR and Cubic spline models for a selection of nuclides. The models have been trained on a squared grid with a spacing of 4 units. Highlighted cells indicate smallest error in the comparison. RMSE values are in Kg}
        \label{res:grid4}
\end{table}


==> Paper GPR - Annals of Nuclear Energy (Publishing)/Sections/Tables/tableruntime.tex <==
\begin{table*}[ht]
    \centering
    \begin{tabular}{c c c c c}\toprule
    \textbf{Configuration} & \textbf{Cubic Spline}  & \textbf{GPR}$-\mu$ & \textbf{GPR}$-\sigma$ & \textbf{GPR Total} \\
    & [s] &[s] &[s] &[s] \\ \midrule
   %Checkerboard & 1.61e-04 & 4.47e-04 & 6.13e-04  & 1.06e-03\\
   Scenario A & 3.40e-05 & 4.61e-04 & 6.00e-04 & 1.06e-03  \\
   %Grid - Spacing 4 & 3.03e-06 & 3.64e-04 & 3.17e-04 & 6.82e-04 \\ 
   Scenario B & 9.74e-06 & 1.18e-03& 9.95e-04& 2.18e-03 \\
   \bottomrule
     
    \end{tabular}
    \caption{Run-time comparison for different configurations.} %Reported values are means over regressions performed on all isotopes, therefore the total time for a GPR prediction does not match with the sum of GPR components run-time.}
    \label{tab:runtime}
\end{table*}

==> Paper GPR - Annals of Nuclear Energy (Publishing)/Sections/Tables/tablesobol.tex <==

\begin{table}[ht!]
\centering
	\resizebox{\tablesize\textwidth}{!}{
		\pgfplotstabletypeset[
		multicolumn names, % allows to have multicolumn names
		col sep=comma,
		columns = {Nuclide,mean_isotope,Spline-RMSE,GPR-RMSE,RatioCubicGPR,SplineRsquared,GPRRsquared,GPRPredictionin1sigma},
		columns/Nuclide/.style={
			column name=$Nuclide$, % name of first column
			string type},  % use siunitx for formatting
		columns/mean_isotope/.style={
			column name=$\mu$, % name of first column
			precision=2,fixed}, 
		columns/Spline-RMSE/.style={
			column name= Cubic Spline,
			string type},
		columns/GPR-RMSE/.style={
			column name=$GPR$,string type},
		columns/RatioCubicGPR/.style={
		column name=RMSE $\frac{Spline}{GPR}$,
		precision=2},
		columns/SplineRsquared/.style={
			column name=$R^{2}_{Sp}$,
			%sci, sci zerofill,
			precision=2},%, sci 10e},
		columns/GPRRsquared/.style={
			column name=$R^{2}_{GPR}$,
			%sci, sci zerofill,
			precision=2},%, sci 10e},
		columns/GPRPredictionin1sigma/.style={
			column name=$Pred-1\sigma$,
			precision=1,},
		every head row/.style={
			before row={\toprule}, % have a rule at top
			after row={
							&	Kg& $\mathrm{RMSE}$ & $\mathrm{RMSE}$  & &  & & $\%$ \\%& $\%$ \\ % the units seperated by &
				\midrule} % rule under units
		},
		every last row/.style={after row=\bottomrule}, % rule at bottom
		]{Sections/Tables/Sobol_all_2space.csv} % filename/path to file
		}
			\caption{Comparison between GPR and Cubic spline models for a selection of nuclides. The models have been trained on samples generated from a 2-dimensional 
			Sobol quasirandom sequence. Highlighted cells indicate smallest error in the comparison. RMSE values are in Kg}
	\label{res:sobol}
\end{table}


==> Paper GPR - Annals of Nuclear Energy (Publishing)/Sections/Tables/tablesobolnew.tex <==
\begin{center}
\begin{table*}[ht!]
\centering
	\resizebox{\tablesize\textwidth}{!}{
		\pgfplotstabletypeset[
		multicolumn names, % allows to have multicolumn names
		col sep=comma,
		columns = {Nuclide,mean_isotope,Spline-RMSE,GPR-RMSE,RatioCubicGPR,SplineRsquared,GPRRsquared,GPRPredictionin1sigma},
		columns/Nuclide/.style={
			column name=$Nuclide$, % name of first column
			string type},  % use siunitx for formatting
		columns/mean_isotope/.style={
			column name=$\mu$, % name of first column
			precision=2,fixed}, 
		columns/Spline-RMSE/.style={
			column name= Cubic Spline,
			string type},
		columns/GPR-RMSE/.style={
			column name=$GPR$,string type},
		columns/RatioCubicGPR/.style={
		column name=RMSE $\frac{Spline}{GPR}$,
		precision=2},
		columns/SplineRsquared/.style={
			column name=$1 - R^{2}_{Sp}$,
			%sci, sci zerofill,
			string type},%, sci 10e},
		columns/GPRRsquared/.style={
			column name=$1 - R^{2}_{GPR}$,
			%sci, sci zerofill,
			string type},%, sci 10e},
		columns/GPRPredictionin1sigma/.style={
			column name=$Pred-1\sigma$,
			precision=1,},
		every head row/.style={
			before row={\toprule}, % have a rule at top
			after row={
							&	Kg& $\mathrm{RMSE}$ & $\mathrm{RMSE}$  & &  & & $\%$ \\%& $\%$ \\ % the units seperated by &
				\midrule} % rule under units
		},
		every last row/.style={after row=\bottomrule}, % rule at bottom
		]{Sections/Tables/SobolNew169_Sobol_all_2space.csv} % filename/path to file
		}
			\caption{\textbf{Scenario B:} Comparison between GPR and Cubic spline models for a selection of nuclides. Highlighted cells indicate smallest error in the comparison. RMSE values are in Kg}
	\label{tab:sobolnew}
\end{table*}
\end{center}


==> Paper GPR - Annals of Nuclear Energy (Publishing)/Sections/TheoreticalBackground.tex <==
\section{Creating the datasets}\label{sec:Models}
% Theoretical Description of GP
\subsection{Reactor simulations}
For our research, we have modeled a 2D infinite lattice model of a CANDU 6 reactor based on specifications from available literature \cite{Candu}. The implementation has been made in the computer code \texttt{SERPENT 2} which couples a Monte Carlo neutron transport module with a fuel depletion solver based on the Chebyshev Rational Approximation Method \cite{serpent}. The quality of the model has been examined by comparing end-of-cycle isotopic compositions with the \texttt{Bruce-1} dataset reported in the SFCOMPO-2.0 database \cite{sfcompo}. Figure \ref{fig:2dlattice} shows the CANDU 6 37-elements fuel assembly implemented in \texttt{SERPENT 2}.
% This type of reactor is of further interest for nuclear non proliferation due to its characteristics of online refueling, and natural uranium fuel. These may facilitate undeclared activities such as the production and diversion of weapons grade plutonium, an element of critical importance for international security.

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{Sections/Images/Candu_geom.png}
    \caption{CANDU 6, 37-element fuel assembly, 2D infinite lattice implementation in \texttt{SERPENT 2} (light green indicates the fuel elements, white for the coolant, pink for the calandria and pressure tubes, black for the void between these tubes and turquoise for the moderator between fuel channels)}
    \label{fig:2dlattice}
\end{figure}

\begin{table}[ht]
    \centering
    \begin{tabular}{c c}
        \toprule
        \textbf{Parameters} & \textbf{Range} \\ \midrule
         Moderator Temperature & 333 - 363 $K$ \\
         Burnup & 0.1 - 7 $\frac{\mathrm{MWd}}{\mathrm{kg_{HM}}}$ \\
         \bottomrule
    \end{tabular}
    \caption{Parameter ranges used in in the generation of the training and testing datasets}
    \label{tab:paramranges}
\end{table}



\subsection{Sampling strategies}
Strategies are required to sample sets of input parameters for each Serpent simulation involved in model development and testing. In this study, we sample moderator temperature and discharge burnup. Table \ref{tab:paramranges} indicates the range of values considered for these parameters. 

Previous studies on sampling schemes and strategies have shown that uniform grid sampling performs poorly in higher-dimensional input spaces \cite{DOE}. While a random number sequence can overcome this issue in principle, due to the nature of pseudo-random number generators implementations, random number sequences tend to cluster, resulting in a non-uniform distribution of samples across the input space. In such cases, a quasirandom sequence can provide a set of samples with a better spatial distribution\cite{qsr}

Sobol quasirandom sampling is a method to generate quasi-random sequences which is designed to minimize the star discrepancy, a mathematical term describing the difference between the distribution of values generated by a certain generating scheme to a multidimensional uniform probability distribution. The generation of the samples involves using a special algorithm in which bitwise operations are performed. Details on the algorithm and its implementation can be found in \cite{SobolSQ}.

In order to evaluate the impact of the sampling method on the prediction quality of the models, two scenarios have been prepared.  In Scenario A, a 25x25 2D-grid dataset was used and simulated, based on the parameter ranges of Table \ref{tab:paramranges}. In this scenario a set of 169 samples was generated from the selection of samples starting from the corners and leaving one grid element in between. The rest of the unselected grid points are then considered as the test dataset, for both this and the following scenario. Scenario B consists of 169 samples generated from a Sobol sequence sampler written in-house. Again, the test dataset is the same as for Scenario A. \\ Figure \ref{fig:SvG} shows a comparison between the samples generated via the Sobol sequence and the aforementioned grid. While grid sampling is still effective in two dimensions, the good space coverage of the Sobol sequence is evident. Figure \ref{fig:exppatterns} shows the spatial arrangement of Scenario A's training set through the bright elements, while the darker elements represent the test dataset used for both scenarios. Table \ref{tab:setups} summarizes the different scenarios and their characteristics


\begin{figure}
    \centering
    \input{Sections/Images/sampling_comparison}
    \caption{Comparison between the dataset based on Sobol quasirandom sampling (left) and the dataset based on Grid sampling (right). While both the Sobol sequence and grid sampling are effective in two dimensions as seen here, the Sobol sequence by far outperforms grid sampling in higher dimensions, at the same number of samples.}
    \label{fig:SvG}
    
\end{figure}

%---------------------------------
% To study the impact of the spatial arrangement of the training data on the model's quality assessed from the test data, both taken from the first dataset, we have consider two setups. The first consists on a grid pattern with a spacing of one cell superimposed on the original 25x25 grid. (see Figure \ref{fig:exppatterns}). In the case of the second dataset, the training set will consist of the samples generated by the Sobol sequence, while the test set corresponds to the entire first dataset done on the 25x25 grid. This approach a direct comparison between Cubic Splines and Gaussian Process based models on two different sampling strategies (see Table \ref{tab:setups}).

\begin{figure}
    \centering
%    \includegraphics[width=0.32\textwidth,trim=2cm 1.3cm 2cm 1.4cm, clip]{Sections/Images/checkerboard.pdf}
    \includegraphics[width=0.32\textwidth,trim=2cm 1.3cm 2cm 1.4cm, clip]{Sections/Images/grid2.pdf}
   % \includegraphics[width=0.32\textwidth,trim=2cm 1.3cm 2cm 1.4cm, clip]{Sections/Images/grid4.pdf}
    \caption{Spatial distribution pattern used to evaluate the performance of the surrogate models on a grid. The yellow elements represent the simulations to be used for training the interpolators, while the dark regions represent the cells where the values will be interpolated.
    }
    \label{fig:exppatterns}
\end{figure}

\begin{table}[ht]
    \centering
    \begin{tabular}{c c c}
    \toprule
     \textbf{Configuration}&\textbf{Training set size}  & \textbf{Test set size}   \\ \midrule
     Scenario A& 169 (Grid)  & 456 (Grid)   \\
     Scenario B & 169 (Sobol) & 456 (Grid) \\
     %Grid - Spacing 4*& 49  & 576    \\
     %Checkerboard& 313 & 312  \\
     
    \bottomrule 
    \end{tabular}
    \caption{Details of the sampling strategies. The different configurations allow for the study of model performance under varying spatial sample distributions}
    \label{tab:setups}
\end{table}

\section{Building the model}
\label{sec:Reg}

Based on the pre-generated training data, we built the Cubic Spline and the GPR models. In the following section we examine these methods.

\subsection{Cubic Spline Interpolation}
% Theoretical Description of Cubic-Spline
Cubic Spline Interpolation is a method to interpolate functions within the boundaries described by a number of its samples. The interpolation procedure consists of fitting a piecewise cubic polynomial between the sampled points. This method results in smoother and higher quality interpolators in comparison to methods such as Langrange and Newton polynomial fitting \cite{NM2}. In addition, it has the advantage of avoiding oscillations and Runge's phenomenon. A more detailed description of the method and its implementation can be found in \cite{CSplines}.

%The former consists of fitting a piecewise cubic polynomial between the sampled points \cite{na}.  
%This method results in smoother and higher quality interpolators in comparison to methods such as Langrange and Newton polynomial fitting \cite{na}. In addition, it has the advantage of avoiding oscillations and Runge's phenomenon. 
%We have used the \texttt{SmoothBivariateSpline} module from the \texttt{Scipy} python package. The latter is discussed in the following.

\subsection{Gaussian Process Regression}

A GP is a set of random variables that share a joint Gaussian probability distribution. GP's can be used for the construction of probabilistic surrogate models of black-box problems where an analytical form is unavailable or intractable and the computational cost is elevated. Without loss of generalization, the aim of GPR is to approximate a function $Y(\vv{X}),\, \vv{X} = (x_{1},..., x_{d})$ through a GP as:
\begin{equation}
    Y(\vv{X}) \approx \mathcal{G}\mathcal{P}(\vv{X}) = \mathcal{N}(0,K(\vv{X}))
\end{equation}
Where $d$ is the dimension of the input space. The kernel ($K$) of a GP is a function which describes the covariance between the inputs of the target function. It encodes a limited set of assumptions about the underlying function such as smoothness and differentiability. By choosing a kernel, an infinite set of functions which share the kernel properties are used to perform the regression, and by training the kernel parameters based on the input and output data a subset of those functions are chosen that match the data.
We chose the Anisotropic Squared Exponential (ASE) kernel, which provides for very smooth interpolation and is infinitely differentiable, as we expect that the change of nuclide concentrations throughout the parameter space would meet these characteristics. An additional advantage is that the ASE kernel allows for the determination of relative input parameter relevance through the use of different correlation lengths parameters ($\ell_{i}$) for each input:

\begin{equation}\label{eq:ASE}
    K(\vv{X},\vv{Z}) = exp\left(-\sum_{i}^{d}\left( \dfrac{x_{i}-z_{i} } {\ell_{i}}\right)^{2}\right)
\end{equation}
Where $\vv{X},\vv{Z}$ are two different points in which the covariance function is evaluated. The smaller $\ell_{i}$, the more sensitive the underlying model is to changes in input $x_{i}$. Once the parameters of the kernel that reproduce the training data are estimated, the posterior predictive distribution of the GP - our model - at an unseen point ($*$) is given by a normal distribution with prediction mean ($\mu_{*}$), prediction variance ($\sigma^{2}_{*}$) and prediction gradient ($\nabla\mu_{*}$):
\begin{align}
    \mu_{*} &= K_{train,*}  (K_{train,train})^{-1} Y_{train} \nonumber \\
    \sigma^{2}_{*} &= K_{*,*} - K_{*,train}^{T}(K_{train,train})^{-1}K_{*,train} \nonumber \\
    \nabla\mu_{*} &= \nabla K_{train,*}  (K_{train,train})^{-1} Y_{train}
\end{align}
    
 To implement the GPR models, we have used the \texttt{scikit-learn} Python package \cite{scikit-learn}. More details on GP's and their kernels can be found in \cite{6}. 

%The choice of kernel will impact the output of the surrogate model, however it remains subject to the user's judgement and knowledge of the process under analysis.

\subsection{Cross-validation}

Since the kernel training process is strongly dependent on the training data, weak prediction performance can occur if an inappropriate selection of the training set is made. This can be avoided by cross-validation.
% which aims to better tune the parameters of a model in order to improve prediction accuracy and precision. %(the last one is not the word i'm looking for)
It is implemented by splitting the training set into k ``folds'' of approximately equal size and performing the training on each fold, thus obtaining the model parameters, then using the other folds as test data to evaluate the model predictive quality. 

This should be performed several times by randomizing the selection of the folds, thus generating a set of plausible model parameters from which the best performing combinations can be selected. Notwithstanding this, a major benefit of cross-validation is that it allows the training of models with different combinations of samples spanning the entire input space, providing parameter sets that tend to enhance the model generalization properties, typically at a smaller computational cost since the training set size is reduced. 

Each \texttt{SERPENT 2} simulation provides an output vector containing about 1300 nuclides. We have created GPR models for each of these nuclides for both datasets. Each GPR model has been trained using a 5-fold cross validation scheme that has been repeated 10 times, thus generating a set of 50 kernel parameter combinations from which the best-performing is chosen. Figures \ref{fig:gpr_model}, \ref{fig:sr90} and \ref{fig:eu154} show the computed GPR models for $^{239}$Pu, $^{90}$Sr and $^{154}$Eu respectively. The models shown are based on the Sobol sequence dataset from scenario B.

\begin{figure}
    \centering
    \resizebox{.95\textwidth}{!}{
    \input{Sections/Images/Pu2d}
    \input{Sections/Images/Pu1d}
    }
    \caption{Reconstruction plots for $^{239}$Pu. The left plot shows the GPR model based on samples generated by the Sobol sequence, showing the mass as a function of burnup and temperature. The reported masses have been scaled by the number of fuel assemblies in the reactor and their dimensions. The squares indicate the samples obtained from the Sobol sequence. The plot on the right shows the same model but plotting this time the predictions for two fixed temperature values alongside their posterior uncertainties. The latter are shown at the 6-$\sigma$ level. %The test points stem from grid sampling and show the accuracy of the model. 
    	A portion of the high burnup section of the plot has been zoomed in in the top left corner, making evident the small albeit important effect of temperature at higher burnups. A lower temperature results in more plutonium being produced. This can be explained by a thermal broadening of $^{238}$U resonances. Below this plot, the errors of both curves is shown. It can be observed that they are distributed around zero.}
    \label{fig:gpr_model}
\end{figure}


% I think that the 1d plot looks very small, and therefore it makes sense to plot the deviation from the prediction, that way the uncertainty can be better appreciated.















==> Sections/Sections/Images/Pu2d.tex <==
	\newcommand{\dsurfPu}{Sections/Images/2dSobolPu239.csv}
	\newcommand{\dsurfPuN}{Sections/Images/Pu2392dComplement.csv}	
	\begin{axis}[name = surf,
		%at=(collapsed.right of south east) ,anchor=left of south west,
		smooth,
		legend pos = north east,
		%mark repeat=10,%
		colormap/greenyellow,
		xlabel = {\textbf{Temperature} ($K$ )},
		ylabel = \textbf{Burnup} $\frac{\mathrm{MWd}}{\mathrm{KgHM}}$,
		zlabel = \textbf{Mass} (Kg),
		xlabel style={rotate=-9},
		ylabel style={rotate=35},  title= $^{239}$\textbf{Pu}
		%y label/.append style={at=(ticklabel* cs:0)},
		%zlabel style={anchor=south west},] %
		]
		\addplot3 [surf,z buffer=sort, mesh/rows=25, opacity=0.6]
		table[y={Burnup}, x={Temperature} , z={Pred}, col sep=comma] {\dsurfPu};
		\addplot3+[only marks, scatter] table[y={Burnup}, x={Temperature} , z={Yts}, col sep=comma] {\dsurfPuN};
	\end{axis} %

==> Sections/Tables/tablecheckerboard.tex <==

\begin{table}[ht!]
\centering
	\resizebox{\tablesize\textwidth}{!}{
		\pgfplotstabletypeset[
		multicolumn names, % allows to have multicolumn names
		col sep=comma, % the seperator in our .csv file
		columns = {Nuclide,mean_isotope,Spline-RMSE,GPR-RMSE,RatioCubicGPR,SplineRsquared,GPRRsquared,GPRPredictionin1sigma},
		columns/Nuclide/.style={
			column name=$Nuclide$, % name of first column
			string type},  % use siunitx for formatting
		columns/mean_isotope/.style={
			column name=$\mu$, % name of first column
			precision=2,fixed}, 
		columns/Spline-RMSE/.style={
			column name= Cubic Spline,
			string type},
		columns/GPR-RMSE/.style={
			column name=$GPR$,string type},
		columns/RatioCubicGPR/.style={
		column name=RMSE $\frac{Spline}{GPR}$,
		precision=2},
		columns/SplineRsquared/.style={
			column name=$R^{2}_{Sp}$,
			%sci, sci zerofill,
			precision=2},%, sci 10e},
		columns/GPRRsquared/.style={
			column name=$R^{2}_{GPR}$,
			%sci, sci zerofill,
			precision=2},%, sci 10e},
		columns/GPRPredictionin1sigma/.style={
			column name=$Pred-1\sigma$,
			precision=1,},
		%display columns/8/.style={
		%	column name=$Pred-2\sigma$,
		%	precision=1,},
		every head row/.style={
			before row={\toprule}, % have a rule at top
			after row={
							&	Kg& $\mathrm{RMSE}$ & $\mathrm{RMSE}$  & &  & & $\%$ \\% & $\%$ \\ % the units seperated by &
				\midrule} % rule under units
		},
		every last row/.style={after row=\bottomrule}, % rule at bottom
		]{Sections/Tables/Checkerboard_all_2space.csv} % filename/path to file
		}
			\caption{Comparison between GPR and Cubic spline models for a selection of nuclides. The models have been trained on a squared grid with a Checkerboard arrangement. Highlighted cells indicate smallest error in the comparison. RMSE values are in Kg}
        \label{res:checkerboard}
\end{table}


==> Sections/Tables/tablegrid4.tex <==

\begin{table}[ht!]
\centering
    \resizebox{\tablesize\textwidth}{!}{
		\pgfplotstabletypeset[
		multicolumn names, % allows to have multicolumn names
		col sep=comma, % the seperator in our .csv file
		columns = {Nuclide,mean_isotope,Spline-RMSE,GPR-RMSE,RatioCubicGPR,SplineRsquared,GPRRsquared,GPRPredictionin1sigma},
		columns/Nuclide/.style={
			column name=$Nuclide$, % name of first column
			string type},  % use siunitx for formatting
		columns/mean_isotope/.style={
			column name=$\mu$, % name of first column
			precision=2,fixed}, 
		columns/Spline-RMSE/.style={
			column name= Cubic Spline,
			string type},
		columns/GPR-RMSE/.style={
			column name=$GPR$,string type},
		columns/RatioCubicGPR/.style={
		column name=RMSE $\frac{Spline}{GPR}$,
		precision=2},
		columns/SplineRsquared/.style={
			column name=$R^{2}_{Sp}$,
			%sci, sci zerofill,
			precision=2},%, sci 10e},
		columns/GPRRsquared/.style={
			column name=$R^{2}_{GPR}$,
			%sci, sci zerofill,
			precision=2},%, sci 10e},
		columns/GPRPredictionin1sigma/.style={
			column name=$Pred-1\sigma$,
			precision=1,},
		every head row/.style={
			before row={\toprule}, % have a rule at top
			after row={
							&	Kg& $\mathrm{RMSE}$ & $\mathrm{RMSE}$  & &  & & $\%$ \\%& $\%$ \\ % the units seperated by &
				\midrule} % rule under units
		},
		every last row/.style={after row=\bottomrule}, % rule at bottom
		]{Sections/Tables/Even_all_4space.csv} % filename/path to file
		}
			\caption{Comparison between GPR and Cubic spline models for a selection of nuclides. The models have been trained on a squared grid with a spacing of 4 units. Highlighted cells indicate smallest error in the comparison. RMSE values are in Kg}
        \label{res:grid4}
\end{table}


==> Sections/Tables/tablesobol.tex <==

\begin{table}[ht!]
\centering
	\resizebox{\tablesize\textwidth}{!}{
		\pgfplotstabletypeset[
		multicolumn names, % allows to have multicolumn names
		col sep=comma,
		columns = {Nuclide,mean_isotope,Spline-RMSE,GPR-RMSE,RatioCubicGPR,SplineRsquared,GPRRsquared,GPRPredictionin1sigma},
		columns/Nuclide/.style={
			column name=$Nuclide$, % name of first column
			string type},  % use siunitx for formatting
		columns/mean_isotope/.style={
			column name=$\mu$, % name of first column
			precision=2,fixed}, 
		columns/Spline-RMSE/.style={
			column name= Cubic Spline,
			string type},
		columns/GPR-RMSE/.style={
			column name=$GPR$,string type},
		columns/RatioCubicGPR/.style={
		column name=RMSE $\frac{Spline}{GPR}$,
		precision=2},
		columns/SplineRsquared/.style={
			column name=$R^{2}_{Sp}$,
			%sci, sci zerofill,
			precision=2},%, sci 10e},
		columns/GPRRsquared/.style={
			column name=$R^{2}_{GPR}$,
			%sci, sci zerofill,
			precision=2},%, sci 10e},
		columns/GPRPredictionin1sigma/.style={
			column name=$Pred-1\sigma$,
			precision=1,},
		every head row/.style={
			before row={\toprule}, % have a rule at top
			after row={
							&	Kg& $\mathrm{RMSE}$ & $\mathrm{RMSE}$  & &  & & $\%$ \\%& $\%$ \\ % the units seperated by &
				\midrule} % rule under units
		},
		every last row/.style={after row=\bottomrule}, % rule at bottom
		]{Sections/Tables/Sobol_all_2space.csv} % filename/path to file
		}
			\caption{Comparison between GPR and Cubic spline models for a selection of nuclides. The models have been trained on samples generated from a 2-dimensional 
			Sobol quasirandom sequence. Highlighted cells indicate smallest error in the comparison. RMSE values are in Kg}
	\label{res:sobol}
\end{table}

